Stoch BiRo: Design and Control of a low cost bipedal robot

This paper introduces the Stoch BiRo, a cost-effective bipedal robot designed with a modular mechanical structure having point feet to navigate uneven and unfamiliar terrains. The robot employs proprioceptive actuation in abduction, hips, and knees, leveraging a Raspberry Pi4 for control. Overcoming computational limitations, a Learning-based Linear Policy controller manages balance and locomotion with only 3 degrees of freedom (DoF) per leg, distinct from the typical 5DoF in bipedal systems. Integrated within a modular control architecture, these controllers enable autonomous handling of unforeseen terrain disturbances without external sensors or prior environment knowledge. The robot's policies are trained and simulated using MuJoCo, transferring learned behaviors to the Stoch BiRo hardware for initial walking validations. This work highlights the Stoch BiRo's adaptability and cost-effectiveness in mechanical design, control strategies, and autonomous navigation, promising diverse applications in real-world robotics scenarios.

==> Reinforcement_Learning_Framework.tex <==
Our approach centers on sim-to-real reinforcement learning (RL) to cultivate bipedal locomotion skills, assuming a foundational understanding of RL \cite{sutton2018reinforcement}. In the broader RL framework, the robot's control policy $\pi$ operates discretely at each time step \(t\), taking in the current state \(s_t\) and producing an action \(a_t\). Executing this action leads to a transition to the subsequent state \(s_{t+1}\). The dynamics governing these state transitions remain unknown to the robot, influenced by environmental conditions such as terrain type and the inherent dynamics of the robot itself. As the learning process unfolds, each state transition corresponds to a real-valued reward \(r_t\), strategically aligned with predefined goals to incentivize desired behavior. Our RL optimization objective revolves around learning a policy that, through dynamic interaction with the environment, maximizes the expected cumulative discounted reward over a finite horizon \(T\). Formally, our goal is to discover a policy $\pi$ that maximizes the objective function: \(J(\pi) = \mathbb{E} \sum_{t=0}^{T} \gamma^t R_t\), where \(\gamma \in [0, 1]\) represents the discount factor, and \(R_t\) serves as a random variable denoting the reward at time \(t\) when following $\pi$ from a state drawn from an initial state distribution.



==> system_architecture.tex <==
\subsection{Computing and Low-Level Control Architecture}
The biped robot model comprises 6 floating Degrees of Freedom (DoF) and 6 actuated DoF. Specifically designed actuators, incorporating high torque density motors and a 9:1 gear reduction, are adept at monitoring joint angles and torques through the utilization of joint encoders and current sensors. The Stoch BiRo incorporates a layered computing architecture, that enhances its control mechanisms for both locomotion and state estimation. This architecture is designed to ensure low-level leg and motor control operates at higher loop frequencies than locomotion control, promoting agility and responsiveness. Moreover, it enables effortless scalability of computational resources to accommodate forthcoming needs in sensing, planning, and navigation. The central processing hub of the Stoch BiRo is a Raspberry Pi 4, functioning on a Linux-based operating system. This component utilizes its computational prowess for executing tasks related to locomotion control and state estimation. The processor communicates through a Pi3Hat daughter board to MJBOTS moteus r4.11 drivers on each actuator via a 5Mbps CAN interface with each leg in a single CAN bus. This setup executes control strategies, including joint PD control at 200 Hz.


